Cost-sensitive Hierarchical Clustering for Dynamic Classifier Selection

We consider the dynamic classifier selection (DCS) problem: Given an ensemble of classifiers, we are to choose which classifier to use depending on the particular input vector that we get to classify. The problem is a special case of the general algorithm selection problem where we have multiple different algorithms we can employ to process a given input. We investigate if a method developed for general algorithm selection named cost-sensitive hierarchical clustering (CSHC) is suited for DCS. We introduce some additions to the original CSHC method for the special case of choosing a classification algorithm and evaluate their impact on performance. We then compare with a number of state-of-the-art dynamic classifier selection methods. Our experimental results show that our modified CSHC algorithm compares favorably

==> benchmarks_LP_recourse.tex <==
\begin{tabular}{|c|r|r|r|r||r|r|}
\toprule
\hline
 \bf  &  \bf    CSHC & \bf  *-RR & \bf *-LP & \bf *-LPR & Best Base & Oracle \\ \hline\hline
\midrule
balance-scale   &   \bf 90.3    &       \bf 90.3        &  \bf  90.3            &  \bf  90.3            & 91.30 & 93.24  \\
bank-marketing  &   \bf 89.7    &       \bf  89.5       &       89.4            & \bf    89.5           & 89.62 & 96.49  \\
Bioresponse     &        74.4   &          75.4         &  \bf 75.8             &  \bf   75.8           & 74.31 & 93.70  \\
breast-w        &   \bf 97.4    &   97.0                &  \bf 97.4             &   97.0                & 96.97 & 98.70  \\
cmc             &   \bf 52.2    &   \bf  51.1           &          49.9         & \bf     51.3          & 51.54 & 85.22  \\
cnae-9          &   86.6        &   88.0                &  \bf 89.1             &   88.0                & 86.55 & 96.64  \\
credit-approval &   86.0        &    \bf  89.0          &   88.6                &      88.6             & 88.60 & 95.61 \\
credit-g        &   \bf 75.2    &          74.5         &   74.5                &    \bf  75.2          & 73.33 & 94.85 \\
diabetes        &   74.8        &   \bf 76.4                &   74.8                &     75.2          & 75.98 & 89.76 \\
eeg-eye-state   &   93.0        &   90.1                &   \bf 93.1            &  \bf   93.1           & 93.10 & 99.90 \\
eucalyptus      &   58.8        &  \bf 62.6             &  60.5                 &    61.7               & 61.32 & 86.42 \\
gina\_agnostic  &    \bf 89.3   &   88.6                &  \bf 89.3             &   \bf  89.3           & 89.34 & 97.99 \\
heart-h         &   \bf 81.6    &   80.6                &  80.6                 &     80.6              & 81.63 & 89.80  \\
hill-valley     &   51.5        &   52.5                &   52.2                & \bf    53.8           & 45.75 & 97.25  \\
ilpd            &   70.5        &   71.0                &  \bf 72.5             &  \bf   72.5           & 70.98 & 98.96 \\
isolet          &   94.8        &   94.6                &  \bf 94.9             &  \bf  94.9            & 94.79 & 98.60  \\
kc1             &   84.9        &  \bf 86.1             & 85.2                  &   85.1                & 85.92 & 93.97  \\
kc2             &   80.3        &  \bf 83.8             &  81.5                 &    83.2               & 84.97 & 91.91  \\
kr-vs-kp        &   98.4    &   98.0                &  \bf 98.5             &    98.4           & 97.91 & 100.0 \\
letter          &   93.0        &   93.3                &  \bf 93.4             &  \bf  93.4            & 92.20 & 97.53 \\
mfeat-factors   &   95.8        &   96.4                &  \bf 96.5             &  96.2                 & 95.91 & 98.71 \\
mfeat-fourier   &   79.5        &   80.6                &   \bf 80.9            &   80.3                & 80.15 & 93.94 \\
mozilla4        &   \bf 92.4    &   90.1                &   92.2                &      92.3             & 80.72 & 98.27 \\
musk            &  \bf 100.0    &  \bf 100.0            &  \bf 100.0            &  \bf  100.0           & 100.0 & 100.0 \\
nomao           &   95.5        &   95.7                &  \bf 95.8             &  95.7                 & 95.52 & 99.22 \\
optdigits       &   98.2        &   98.2                &  \bf 98.3             &  \bf 98.3             & 98.11 & 99.62 \\
ozone-level-8hr &   92.6        &   \bf 93.1            &  \bf 93.1             &   92.7                & 93.17 & 98.57 \\
pc1             &   \bf 95.6    &   \bf  95.6           &  95.4                 &  \bf 95.6             & 95.08 & 97.81 \\
pc3             &   \bf 90.1    &   89.5                &  89.0                 &   89.5                & 90.50 & 95.35 \\
pendigits       &   \bf 99.3    &   99.2                &   \bf 99.3            & \bf    99.3           & 99.26 & 99.72 \\
phoneme         &   84.4        &  \bf  86.0            &  85.2                 &    85.4               & 85.09 & 97.81 \\
qsar-biodeg     &    84.2       &   84.2                &  \bf 85.7             &    85.1               & 85.39 & 96.56 \\
scene           &    95.5       &    95.5               &  84.5                 & \bf     96.0          & 94.47 & 99.50 \\
spambase        &   93.7        &    94.1               &  \bf 95.7             &     94.1              & 93.42 & 99.28 \\
SpeedDating     &   85.1        &   85.4                &   \bf 94.1            &     85.4              & 85.18 & 97.03 \\
splice          &   91.6        &  \bf  93.3            &   93.2                &     93.0              & 91.74 & 98.48 \\
tic-tac-toe     &   85.8        &   86.1                &   86.8                &     \bf 87.1          & 84.23 & 97.48 \\
vehicle         &   73.6        &  \bf  77.1            &  76.8                 &  \bf 77.1             & 75.00 & 92.14 \\
vowel           &   83.5    &   82.6                &  \bf 85.6             &    84.4           & 85.02 & 94.50 \\
wdbc            &    97.9       &   96.3                &   97.9                &    \bf 98.4           & 97.34 & 99.47 \\
\bottomrule
\hline\hline
\# losses w.r.t *-LPR &   27.0  &   18.0 &   15.0 &       0.0 & & \\hline
\# wins w.r.t *-LPR   &    6.0  &   10.0 &   13.0 &       0.0 & & \\  \hline
MGI                  &  100.8  &  100.3 &  100.2&     100.0  & &\\ \hline
rank                 &    6.0&    5.6 &    5.2  &       5.1  & &\\  \hline
\hline
\end{tabular}


==> cshc.variants.tex <==
\begin{tabular}{|r|r|r|r|r|}
\toprule
\hline
 \bf  &  \bf    CSHC & \bf  *-RR & \bf *-LP & \bf *-LPR \\ \hline\hline
\midrule
balance-scale   &   \bf 90.3    &       \bf 90.3        &  \bf  90.3            &  \bf  90.3    \\ \hline
bank-marketing  &   \bf 89.7    &       \bf  89.5       &       89.4            & \bf    89.5   \\ \hline
Bioresponse     &        74.4   &          75.4         &  \bf 75.8             &  \bf   75.8   \\ \hline
breast-w        &   \bf 97.4    &   97.0                &  \bf 97.4             &   97.0        \\ \hline
cmc             &   \bf 52.2    &   \bf  51.1           &          49.9         & \bf     51.3  \\ \hline
cnae-9          &   86.6        &   88.0                &  \bf 89.1             &   88.0        \\ \hline
credit-approval &   86.0        &    \bf  89.0          &   88.6                &      88.6     \\ \hline
credit-g        &   \bf 75.2    &          74.5         &   74.5                &    \bf  75.2  \\ \hline
diabetes        &   74.8        &   \bf 76.4                &   74.8                &     75.2      \\ \hline
eeg-eye-state   &   93.0        &   90.1                &   \bf 93.1            &  \bf   93.1   \\ \hline
eucalyptus      &   58.8        &  \bf 62.6             &  60.5                 &    61.7       \\ \hline
gina\_agnostic  &    \bf 89.3   &   88.6                &  \bf 89.3             &   \bf  89.3   \\ \hline
heart-h         &   \bf 81.6    &   80.6                &  80.6                 &     80.6      \\ \hline
hill-valley     &   51.5        &   52.5                &   52.2                & \bf    53.8   \\ \hline
ilpd            &   70.5        &   71.0                &  \bf 72.5             &  \bf   72.5   \\ \hline
isolet          &   94.8        &   94.6                &  \bf 94.9             &  \bf  94.9    \\ \hline
kc1             &   84.9        &  \bf 86.1             & 85.2                  &   85.1        \\ \hline
kc2             &   80.3        &  \bf 83.8             &  81.5                 &    83.2       \\ \hline
kr-vs-kp        &   98.4    &   98.0                &  \bf 98.5             &    98.4       \\ \hline
letter          &   93.0        &   93.3                &  \bf 93.4             &  \bf  93.4    \\ \hline
mfeat-factors   &   95.8        &   96.4                &  \bf 96.5             &  96.2         \\ \hline
mfeat-fourier   &   79.5        &   80.6                &   \bf 80.9            &   80.3        \\ \hline
mozilla4        &   \bf 92.4    &   90.1                &   92.2                &      92.3     \\ \hline
musk            &  \bf 100.0    &  \bf 100.0            &  \bf 100.0            &  \bf  100.0   \\ \hline
nomao           &   95.5        &   95.7                &  \bf 95.8             &  95.7         \\ \hline
optdigits       &   98.2        &   98.2                &  \bf 98.3             &  \bf 98.3     \\ \hline
ozone-level-8hr &   92.6        &   \bf 93.1            &  \bf 93.1             &   92.7        \\ \hline
pc1             &   \bf 95.6    &   \bf  95.6           &  95.4                 &  \bf 95.6     \\ \hline
pc3             &   \bf 90.1    &   89.5                &  89.0                 &   89.5        \\ \hline
pendigits       &   \bf 99.3    &   99.2                &   \bf 99.3            & \bf    99.3   \\ \hline
phoneme         &   84.4        &  \bf  86.0            &  85.2                 &    85.4       \\ \hline
qsar-biodeg     &    84.2       &   84.2                &  \bf 85.7             &    85.1       \\ \hline
scene           &    95.5       &    95.5               &  84.5                 & \bf     96.0  \\ \hline
spambase        &   93.7        &    94.1               &  \bf 95.7             &     94.1      \\ \hline
SpeedDating     &   85.1        &   85.4                &   \bf 94.1            &     85.4      \\ \hline
splice          &   91.6        &  \bf  93.3            &   93.2                &     93.0      \\ \hline
tic-tac-toe     &   85.8        &   86.1                &   86.8                &     \bf 87.1  \\ \hline
vehicle         &   73.6        &  \bf  77.1            &  76.8                 &  \bf 77.1     \\ \hline
vowel           &   83.5    &   82.6                &  \bf 85.6             &    84.4       \\ \hline
wdbc            &    97.9       &   96.3                &   97.9                &    \bf 98.4   \\ \hline
\bottomrule
\hline\hline
\# losses w.r.t *-LPR &   27.0  &   18.0 &   15.0 &       0.0 \\hline
\# wins w.r.t *-LPR   &    6.0  &   10.0 &   13.0 &       0.0 \\  \hline
MGI                  &  100.8  &  100.3 &  100.2&     100.0 \\ \hline
rank                 &    6.0&    5.6 &    5.2  &       5.1 \\  \hline
\hline
\end{tabular}

